Dueling Bandits with Team Comparisons

We introduce the dueling teams problem, a new online-learning setting in which the learner observes noisy comparisons of disjoint pairs of $k$-sized teams from a universe of $n$ players. The goal of the learner is to minimize the number of duels required to identify, with high probability, a Condorcet winning team, i.e., a team which wins against any other disjoint team (with probability at least $1/2$). Noisy comparisons are linked to a total order on the teams. We formalize our model by building upon the dueling bandits setting (Yue et al.2012) and provide several algorithms, both for stochastic and deterministic settings. For the stochastic setting, we provide a reduction to the classical dueling bandits setting, yielding an algorithm that identifies a Condorcet winning team within $\mathcal{O}((n + k \log (k)) \frac{\max(\log\log n, \log k)}{\Delta^2})$ duels, where $\Delta$ is a gap parameter. For deterministic feedback, we additionally present a gap-independent algorithm that identifies a Condorcet winning team within $\mathcal{O}(nk\log(k)+k^5)$ duels.

==> src/distinguish.tex <==



%TODO: Mention that we are in deterministic setting! 

In the previous sections we have seen that witnesses are crucial to our algorithms in order to identify pairwise relations between individual players. Within Section \ref{sec:stochastic} and Section \ref{subsec:alg1}, in order to find out about the relation between two players $a$ and $b$, we have mostly sampled witnesses from the set of all potential witnesses, i.e., $\mathcal{S}_{a,b}$. In Section \ref{subsec:graph-algo} we have used the fact that every pair of disjoint teams $(A,B)$ with $A \succ B$ indeed contains a witness $(S,S')$ with $S \subseteq A$ and $S' \subseteq B$ which shows the relation between some $a \in A$ and $b \in B$. However, this approach comes at the cost of not being able to control for which $a \in A$ and which $b \in B$ the relation is uncovered. Hence, a natural question is whether there exists a smarter way to construct witnesses, without simply sampling them. 

Within this section we present an algorithm that is able to construct a witness that is \emph{universal}. We say that a tuple $(S,S'), |S|=|S'|=k-1, S \cap S'$ is universal, if, for any two nodes $a,b \in [n] - S - S'$, the tuple $(S,S')$ is a witness for the relationship between $a$ and $b$, i.e., $Z_{a,b}(S,S') \in \{0,1\}$. 

However, in order to derive this result, we will need to make one additional assumption about the linear order among the teams. More precisely, we require the linear order to be \emph{additive linear}, meaning that there exist values $v_a \in \mathbb{R}$ for all players $a \in [n]$ such that \[A \succ B \Leftrightarrow \sum_{a \in A} v_a > \sum_{b \in B} v_b.\] We will also use the shorthand notation $v(A) = \sum_{a \in A} v_a$ for any subset $A \subseteq [n]$. We discuss this restriction in detail within the Supplementary Material and in particular derive a sufficient and necessary condition for when an instance of our problem satisfies this condition. This characterization is inspired by \citet{FPR02a} and based on LP duality. 

Our key observation for the construction of the algorithm is the following. 
\begin{lemma}
Let $S,S' \subseteq [n]$ with $S\cap S' = \emptyset$ and $|S|=|S'|=k-1$. Moreover, let $a,b \in [n] - S - S'$. It holds that $Z_{a,b}(S,S')\in \{0,1\}$ if and only if \[ |v_a - v_b| > |\sum_{s \in S}v_s - \sum_{s' \in S'}v_{s'}| .\]
\end{lemma}

\begin{proof}

\end{proof}

\begin{algorithm}
\begin{algorithmic}\label{alg:witness}
\STATE \textbf{Input:} An instance $([n],\succ)$, where $\succ$ is additive linear
\STATE \textbf{Output:} An optimal witness $(S,S')$
\STATE Choose $(S,S')$ such that $S,S\subseteq[n],$ $|S|=|S'|=k-1, S \cap S' = \emptyset$ randomly
\WHILE{$\exists \; a,b \in V - S - S'$ with $(a,b), (b,a) \not\in D$}
\IF{$Z_{a,b}(S,S') \in \{0,1\}$}
\STATE add $(a,b)$ or $(b,a)$ to $D$\\
\STATE \textbf{go to} next iteration of while loop
\ELSE 
\STATE Order $S=\{s_1,\dots,s_{k-1}\}$, $S'=\{s'_1,\dots,s'_{k-1}\}$
\FOR{$i \in [k-1]$}
\IF{$Z_{s_i,s'_i}(S - \{s_i\} \cup \{a\},S' - \{s'_i\} \cup \{b\}) \in \{0,1\}$}
\STATE add $(s_i,s'_i)$ or $(s'_i,s_i)$ to $D$
\STATE $S \leftarrow S - \{s_i\} \cup \{a\}, S' \leftarrow S' - \{s'_i\} \cup \{b\}$
\STATE \textbf{go to} next iteration of while loop
\ENDIF
\ENDFOR
\STATE $(a',b'), (T,T') \leftarrow uncover(S \cup \{a\},S' \cup \{b\})$\\
\STATE add $(a',b')$ to $D$ (if not existent yet)
%\STATE $T \leftarrow T - \{a,b\} \cup \{a'\}, T' \leftarrow T' - \{a,b\} \cup \{b'\}$
\IF{$Z_{a,b}(T- \{a,b\} \cup \{a'\},T'- \{a,b\} \cup \{b'\}) \in \{0,1\}$}
\STATE add $(a,b)$ or $(b,a)$ to $D$ \\
\ELSE \STATE $S \leftarrow T , S' \leftarrow T'$
\ENDIF
\ENDIF
\ENDWHILE
\STATE \textbf{return} $(S,S')$
\caption{Construct optimal witness}
\end{algorithmic}
\end{algorithm}



\begin{lemma}
Let $S,S' \subseteq [n]$ with $S\cap S' = \emptyset$ and $|S|=|S'|=k-2$. Moreover, let $a,b,c,d\in [n] - S - S'$. If 
\begin{enumerate}[label=(\roman*)]
    \item $Z_{a,b}(S \cup \{c\},S' \cup \{d\})=1/2$, and \label{con:witness1}
    \item $Z_{c,d}(S \cup \{a\},S' \cup \{b\})\in \{0,1\}$,\label{con:witness2}
\end{enumerate}
it follows that \[  |v(S \cup \{a\}) - v(S' \cup \{b\})| < |v(S \cup \{c\}) - v(S' \cup \{d\})|.\]
\end{lemma}

\begin{proof}
We start by defining 
\[\delta_{ab} = v_a-v_{b},\quad \delta_{cd} = v_c-v_d,\quad \delta_S = v(S)-v(S').
\]

In general, each of the conditions $(i)$ and $(ii)$ allow for two sub-cases, leading to four different cases in total. However, if we assume without loss of generality that $Z_{c,d}(S \cup \{a\},S' \cup \{b\}) = 1$, this directly implies that $S \cup \{c\} \cup \{a\} \succ S' \cup \{d\} \cup \{b\}$ and $S \cup \{c\} \cup \{b\} \succ S' \cup \{d\} \cup \{a\}$ holds. As a consequence, $(i)$ implies that $\delta_{cd} > |\delta_{S} + \delta_{ab}|$ and $(ii)$ implies that $\delta_{S} + \delta_{cd} > |\delta_{ab}|$. 

%Each of the conditions $(i)$ and $(ii)$ allow for two sub-cases, leading to four different cases in total. More precisely, $(i)$ implies that either %$S \cup \{c\} \cup \{a\} \succ S' \cup \{d\} \cup \{b\}$ and $S \cup \{c\} \cup \{b\} \succ S' \cup \{d\} \cup \{a\}$ or $S' \cup \{d\} \cup \{a\} \succ S \cup \{c\} \cup \{b\}$ and $S' \cup \{c\} \cup \{b\} \succ S \cup \{c\} \cup \{a\}$. 
%$\delta_{S} + \delta_{cd} > |\delta_{ab}|$ or $-(\delta_{S} + \delta_{cd}) > |\delta_{ab}|$. Similarly, $(ii)$ implies that either $\delta_{cd} > |\delta_{S} + \delta_{ab}|$ or $-\delta_{cd} > |\delta_{S} + \delta_{ab}|.$ By symmetry, we can reduce to two different cases. More precisely, we assume wlog that $\delta_S + \delta_{cd} > |\delta_{ab}|$ holds show the claim for the two sub-cases of $(ii)$.  

Hence, we can rephrase our claim to \[\delta_S + \delta_{cd} = |\delta_S + \delta_{cd}| > |\delta_{S} + \delta_{ab}|.\] 

We distinguish two cases. 

\textbf{Case 1:} $\delta_S + \delta_{ab} > 0$. Then it remains to show that $\delta_{cd} > \delta_{ab}$. First, assume $\delta_{S} > 0$. Then, by the implication of $(i)$ we get that $\delta_{cd} > \delta_S + \delta_{ab} > \delta_{ab}$. Second, assume that $\delta_{S}<0$. Then, we get by the implication of $(ii)$ that $\delta_{cd} > \delta_S + \delta_{cd} > \delta_{ab}$. 

\textbf{Case 2:} $\delta_S + \delta_{ab} < 0$. We show that $\delta_S + \delta_{cd} > - (\delta_{S} + \delta_{ab})$. By the implication of $(i)$ and $(ii)$ we get that $\delta_{cd}>0$ and $\delta_{S} + \delta_{cd}>$, respectively. Hence, also 

\end{proof}





The high level idea of the algorithm is the following. 

Remember graph $D$. 
Define graph $G$. 




%Algorithm 


%Proposition
\begin{proposition}
Algorithm \ref{alg:witness} works correctly, i.e., the returned tuple $(S,S')$ is universal. 
\end{proposition}

\begin{proof}
todo. 
\end{proof}

%Proof of proposition
\begin{proposition}
Algorithm \ref{alg:witness} requires $\mathcal{O}(n^2k)$ queries. 
\end{proposition}

\begin{proof}
todo. 
\end{proof}













\iffalse
Idea: First we take two random teams, $A,A'$, with a pair of players $y\in A, y'\in A'$ s.t. 
\[
A_{-y}\cup \{y'\}\prec A'_{-y'}\cup \{y\}
\]
And
\[
A'_{-y}\cup \{y'\}\prec A_{-y}\cup \{y\}
\]
Where the selection of $y,y'$ can be done using the uncover sub-procedure.

Now, try to see whether we can deduce the relation between each pair of ``parallel'' players $x_i\in A, x_i'\in A'$. Let $x,x'$ denote a pair of players for which 
\[
A_{-x}\cup \{x'\}\prec A'_{-x'}\cup \{x\}
\]
And
\[
A'_{-x}\cup \{y'\}\prec A_{-y'}\cup \{y\}
\]

If we can deduce it for any such pair we can replace 

\fi

\newpage 

\begin{claim}
Let $B\cup\{y\},B'\cup\{y'\}$ be two disjoint sets of size $k-1$, and let $x,x'\notin B\cup\{y\}\cup B'\cup\{y'\}$ be two (different) players. Then, if 
\begin{align}\label{eq:By1}
B\cup\{y,x\}\succ B'\cup\{y',x'\},
\end{align}
\begin{align}\label{eq:By2}
B\cup\{y,x'\} \succ B'\cup\{y',x\}
\end{align}
And
\begin{align}\label{eq:y}
B'\cup\{x',y\}\succ B\cup\{x,y'\}
\end{align}

And values of teams are the sums of their players' values, it holds that
\[
|\val{B\cup \{x\}}-\val{B'\cup \{x'\}}|<|\val{B\cup \{y\}}-\val{B'\cup \{y'\}}|.
\]
\end{claim}

\textbf{Counter example for Claim}

Consider the following values: 
\begin{itemize}
    \item $v(B)= v(y') = v(x) = 0$
    \item $v(y) = 21$, $v(B')=v(x')=10$
\end{itemize}

Then, (\ref{eq:By1}) holds since \[v(B) + v(y) + v(x) = 21 > 20 = v(B') + v(y') + v(x'),\]
(\ref{eq:By2}) holds since \[v(B) + v(y) + v(x') = 31 > 10 = v(B') + v(y') + v(x),\]
and (\ref{eq:y}) holds since  \[v(B') + v(y) + v(x') = 31 > 10 = v(B) + v(y') + v(x).\]

However, 
\begin{align*}
&|v(B) + v(x) - v(B') - v(x')| \\
 = &|-10-10| \\
 > &|21-10|\\ 
 = &|v(B) + v(y) - v(B') - v(y')|
\end{align*}



\begin{proof}
First,  denote
\[\alpha_x = \val{x}-\val{x'},\quad \alpha_y = \val{y}-\val{y'},\quad \alpha_B = \val{B}-\val{B'}.
\]

Now, from (\ref{eq:By1}) and (\ref{eq:By2}) and (\ref{eq:y}) we notice that $\alpha_B+\alpha_y>0$, $\alpha_y>0$ hence $|\alpha_B+\alpha_y|=\alpha_B+\alpha_y$ and $|\alpha_y|=\alpha_y$. Overall we get
\begin{equation}\label{eq:1}
|\alpha_B+ \alpha_x|<\alpha_y
\end{equation}
\begin{equation}\label{eq:2}
|\alpha_x|<\alpha_B+\alpha_y.
\end{equation}

We can rephrase the claim as
\[
|\alpha_B+\alpha_x|<\alpha_B+\alpha_y
\]

Now we divide into cases.\\
Case I: $\alpha_x+\alpha_B>0$ (hence $|\alpha_x+\alpha_B|=\alpha_x+\alpha_B$)\\
That means it is sufficient to show that $\alpha_x<\alpha_y$.
If $\alpha_B>0$, it holds because
\[
\alpha_x<\alpha_B+\alpha_x<\alpha_y
\]
Where the first inequality is due to $\alpha_B>0$ and the second is from (\ref{eq:1}).

If $\alpha_B<0$, it holds because
\[
\alpha_x<\alpha_B+\alpha_y<\alpha_y
\]
Where the first inequality is due to (\ref{eq:2}) and the second is from  $\alpha_B<0$.

Case II: $\alpha_x+\alpha_B<0$ (hence $|\alpha_x+\alpha_B|=-\alpha_x-\alpha_B$)\\
From (\ref{eq:2}) we get
\[
0<|\alpha_x|<\alpha_B+\alpha_y
\]
Using (\ref{eq:1}) gives us
\[
0<|\alpha_x|<\alpha_B+\alpha_y<2\alpha_B+\alpha_y+\alpha_x
\]
Subtracting $\alpha_B+\alpha_x$:
\[
|\alpha_B+\alpha_x|=-\alpha_B-\alpha_x<\alpha_B+\alpha_y
\]
As required.
\end{proof}




==> src/improved_deterministic.tex <==



In the following we will assume that $n \in \mathcal{O}(k)$.

We describe an algorithm that finds a Condorcet winning team in $[n]$. We call this algorithm \emph{the cut algorithm}. Crucially, it maintains a partitioning of $[n]$, $\mathcal{T} = \{T_1, \dots, T_{\ell}\}$ for some $\ell \in [n]$ such that \[T_{1} \triangleright T_{2} \triangleright T_{3} \triangleright \dots \triangleright T_{\ell}. \] Recall that $A \triangleright B$ indicates that $a \succ b$ for all $a \in A, b \in B$.   

Before we describe the entire algorithm, we will discuss three subroutines which will play a crucial role within the construction of the algorithm. 

The first subroutine is a variant of \emph{Uncover} and will be used to $(i)$ detect a new relation between $a, b \in T_i$ for some $i \in [\ell]$, or $(ii)$ find a witness for an already known relation $ a\succ b$ for $a \in T_i, b \in T_j, i<j$. 

The second subroutine, \emph{NewCut}, will be called after Uncover was used for purpose $(i)$ and helps to divide $T_i$ into two or three subsets which again form a weak ordering. In other words, \emph{NewCut} refines the partition $\mathcal{T}$. 

Lastly, the subroutine \emph{Compare} is crucial for proving that a candidate team is indeed Condorcet winning. 


\subsection*{Subroutine: WarmstartUncover}

We describe a variant of the uncover subroutine which takes as input four disjoint ordered sets $A,B,C$ and $D$ with $|A|=|B|, |C| = |D|$ and $|A|+|B| =k$.\lc{ have you meant $|A|+|C|=k$?} Moreover, as a requirement, it should hold that $A \cup C \succ B \cup D$ and $A \cup D \succ B \cup C$. As a consequence, we can strengthen the guarantees of the Uncover subroutine, such that for the returned pair and witness $(a,b), (S,S')$ we know that $a$ is from $A$, $b$ is from $B$ and exactly one of $S$ and $S'$ contains $C$ while the other set contains $D$. This will be helpful within the \emph{cut algorithm}. The subroutine is formally described in Algorithm \ref{sub:PartialUncover}. 



\begin{algorithm}[tb] 
\begin{algorithmic}
\STATE \textbf{Input: } four disjoint, ordered subsets of players, $A,B,C,D$ with $|A|=|B|,|C|=|D|, |A| + |C| = k$, $A \cup C \succ B \cup D$, and $ A \cup D \succ B \cup C$\\
\STATE \textbf{Output: } $a \in A, b \in B,$ and $(S,S') \in \mathcal{S}_{a,b}$\lc{, a witness for $a\succ b$} with either ($C \subseteq S$ and $D \subseteq S'$) or ($D \subseteq S$ and $C \subseteq S'$) \\
\smallskip
\STATE Initialize  $S \leftarrow A \cup C$, $T \leftarrow B \cup D$, $\ell \leftarrow 1$, $r \leftarrow |A|$ \\ 
\WHILE{$\ell < r$ }
\STATE $i\leftarrow \big\lfloor\frac{\ell+r}{2}\big\rfloor$\\
\STATE $S\leftarrow S-A_{i+1:r}\cup B_{i+1:r} $\\
\STATE $T\leftarrow T-B_{i+1:r}\cup A_{i+1:r} $\\
\IF{$S \succ T$}
\STATE $r\leftarrow i$
\ELSE \STATE $\ell\leftarrow i+1$ \\ 
\STATE swap $S$ and $T$
\ENDIF
\ENDWHILE
\STATE \textbf{return} $(a_{\ell},b_{\ell}),$ and $(S \setminus \{a_{\ell}\},T \setminus \{b_{\ell}\})$
\end{algorithmic}
\caption{WarmStart Uncover Subroutine}\label{sub:PartialUncover}
\end{algorithm}

\begin{restatable}{lemma}{lemunclog}\label{lem:warmunc-log}
In subroutine WarmStart Uncover (Algorithm \ref{sub:PartialUncover}),
at the end of every while loop, it holds that, $(i) \;\ell, r \in \mathbb{N}$ with $\ell \leq r$, $(ii) \;A_{\ell:r} \subseteq S$, $B_{\ell:r} \subseteq T$, $(iii)\;  S\succ  T$, and $ (iv)\;  T \setminus B_{\ell:r} \cup A_{\ell:r} \succ S \setminus A_{\ell:r} \cup B_{\ell:r}$ $(iv)$ exactly one of $S$ and $T$ contains $C$, the other set contains $D$. 
\end{restatable}

\begin{proof}
$(i)-(iii)$ were proven in the last paper. $(iv)$ is a trivial induction. 
\end{proof}

With the help of Lemma \ref{lem:warmunc-log} it is easy to show the following proposition. 

\begin{restatable}{proposition}{propUncrun}\label{prop:unc-run}
Let $(a_{\ell},b_{\ell}), (S,S')$ be two tuples returned by Algorithm \ref{alg:subroutine}. Then, $a_{\ell} \succ b_{\ell}$ and in particular $(S,S') \in \mathcal{S}_{a,b}$. Moreover, either $C \subseteq S$ and $D \subseteq S'$ or $D \subseteq S$ and $C \subseteq S'$. The running time as well as the number of duels performed by the algorithm are bounded by $\mathcal{O}(\log(|A|))$. 
\end{restatable}

\subsection*{Subroutine: NewCut}

\subsection*{Subroutine: Compare}

The \emph{compare} subroutine is crucial in linking outcomes of duels to differences of (sums of) values. It will be useful in the following situation. Consider a pair of players $(a,b)$ together with a witness
for their relation $(S,S') \in \mathcal{S}_{a,b}$. From this fact, it already follows that $v(a) - v(b) > |v(S) - v(S')|$. However, we will be interested in the question whether a similar relation holds for two subsets of $S$ and $S'$, namely, $C \subseteq S$ and $D \subseteq S'$ of equal size. The \emph{compare} subroutine checks whether such a relation holds by performing two additional duels, namely $(\Bar{S} \cup D \cup \{a\},\Bar{S}' \cup C \cup \{b\})$ and $(\Bar{S}' \cup C \cup \{a\},\Bar{S} \cup D \cup \{b\})$, where $\Bar{S} = S \setminus C$ and $\Bar{S}' = S' \setminus D$. Then, it distinguishes three cases. 

\textbf{Case 1.} $(i)\; \Bar{S} \cup D \cup \{a\} \succ \Bar{S}' \cup C \cup \{b\}$ and $(ii) \;\Bar{S}' \cup C \cup \{a\} \succ \Bar{S} \cup D \cup \{b\}$ 

Recall that from $(S,S') \in \mathcal{S}_{a,b}$ \lc{being a witness for $a\succ b$} we additionally get that $(iii) \; \Bar{S} \cup C \cup \{a\} \succ \Bar{S}' \cup D \cup \{b\}$ and $(iv) \; \Bar{S}' \cup D \cup \{a\} \succ \Bar{S} \cup C \cup \{b\}$ hold. (These also hold for Cases $2$ and $3$.) \lc{I think it's worth mentioning it before we start with the exhaustion.}

In total, from adding $(i)$ and $(iv)$ we get that \[v(a) - v(b)> v(C) - v(D)\]
and from adding $(ii)$ and $(iii)$ we get that 
\[v(a) - v(b) > v(D) - v(C).\]
Summarizing, this yields $v(a) - v(b) >\lc{|v(C)-v(D)|\geq ||v(C)| - |v(D)||\geq } |v(C)| - |v(D)|$\lc{, where the one before last inequality follows from the triangle inequality.}. 

\textbf{Case 2.} $(v) \; \Bar{S}' \cup C \cup \{b\} \succ \Bar{S} \cup D \cup \{a\}$

In that case, observe that the quartet $(C,D,\Bar{S} \cup \{a\}, \Bar{S}' \cup \{b\})$ satisfies the requirements for the \emph{WarmStartUncover} subroutine due to equation $(iii)$ and $(v)$. Hence, \emph{WarmStartUncover} will return a dominance of some player in $C$ towards some player in $D$ together with a witness for this relationship.
\lc{Do you think we should define dominance?}

\textbf{Case 3.} $(vi) \; \Bar{S} \cup D \cup \{b\} \succ \Bar{S}' \cup C \cup \{a\}$

In that case, observe that the quartet $(D,C,\Bar{S} \cup \{b\}, \Bar{S}' \cup \{a\})$ satisfies the requirements for the \emph{WarmStartUncover} subroutine due to equation $(iv)$ and $(vi)$. Hence, \emph{WarmStartUncover} will return a dominance of some player in $C$ towards some player in $D$ together with a witness for this relationship. 



\begin{algorithm}[tb] 
\begin{algorithmic}
\STATE \textbf{Input: } tuple $(a,b)$, witness $(S,S') \in \mathcal{S}_{a,b}$ and $C \subseteq S$, $D \subseteq S'$ with $|C| = |D|$
\STATE \textbf{Output: } \emph{True} (which implies $v(a) - v(b) > |v(C)| - |v(D)|$) or $c \in C$ and $d \in D$ and $(T,T') \in \mathcal{S}_{cd}$\lc{, a witness for $a\succ b$}  %(or $(T,T') \in \mathcal{S}_{dc}$) 
\lc{I commented out the parentheses as $\mathcal{S}_{cd}=\mathcal{S}_{dc}$ and $(T,T')$ is a witness iff $(T',T)$ is a witness} \\
\smallskip
\IF {$S \setminus C \cup D \cup \{a\} \succ S' \setminus D \cup C \cup \{b\}$ and $S' \setminus D \cup C \cup \{a\} \succ S \setminus C \cup D \cup \{b\}$}
\STATE \textbf{return} True
\ELSIF{$S' \setminus D \cup C \cup \{b\} \succ S \setminus C \cup D \cup \{a\} $}
\STATE \textbf{return} $\mathrm{WarmStartUncover}(C,D,S'\setminus D \cup \{b\},S \setminus C \cup \{a\})$
\ELSE \STATE \textbf{return} $\mathrm{WarmStartUncover}(D,C,S\setminus C \cup \{b\},S' \setminus D \cup \{a\})$
\ENDIF
%\STATE \textbf{return} $(a_{\ell},b_{\ell}),$ and $(S \setminus \{a_{\ell}\},T \setminus \{b_{\ell}\})$
\end{algorithmic}
\caption{Compare Subroutine}\label{sub:compare}
\end{algorithm}


\subsection*{Algorithm: CondorcetWinning - Case 1}

Before describing our algorithm formally within Algorithm \ref{alg:condorcet1}, we discuss the main ideas and give some clarifying details. 

The algorithm takes as an input a partition of the players into a weak ordering, i.e., $\mathcal{T} = \{T_1, \dots, T_{\ell}\}$ with $T_1 \triangleright T_2 \triangleright \dots \triangleright T_{\ell}$. We introduce the short-hand notation $T_{\leq j} = \bigcup_{m \in [j]} T_m$ and $T_{< j} = \bigcup_{m\in[j-1]} T_m$ and analogously $T_{\geq j}$ and $T_{> j}$. 

We are especially interested in two indices, namely $i_k \in [\ell]$ such that \[|T_{<i_k}|<k<|T_{\leq i_k}|\] and similarly  $i_{2k} \in [\ell]$ such that \[|T_{<i_{2k}}|<2k<|T_{\leq i_{2k}}|.\] In case one of these indices does not exist, this implies that we have either identified the set $[k]$ or $[2k]$ in which case we can identify a Condorcet winning team. For the sake of brevity we did not include this case within the algorithm yet. Moreover, for now we assume that $i_{k} \neq i_{2k}$ holds. The case $i_{k} = i_{2k}$ is still work in progress. 

\begin{figure}
    \centering
    \includegraphics[scale=.15]{src/figures/fig1.jpg}
    \caption{Caption}
    \label{fig:cut-algo-XY}
\end{figure}

Observe that we already know that $T_{<i_k} \subseteq [k]$ as well as $T_{<i_{2k}} \setminus T_{\leq i_{k}} \subseteq [2k] \setminus [k]$.  



The algorithm will now select a prefix of the weak ordering and either prove that it is a Condorcet Winning team, or refine the weak ordering $\mathcal{T}$ and call itself again. To this end, the set $T_{i_k}$ is first divided into three sets, $X,Y$ and $W$, where $|X|=|Y| = \min \{k-|T_{<i_k}|,|T_{\leq i_k}| - k\}$. As a consequence, $X$ and $Y$ are guaranteed to be non-empty but $W$ can be empty. There are two cases to be distinguished: either $T_{<i_k}$ together with $X$ is already of size $k$ or not. In the first case, set $U = T_{<i_k}$ while in the latter case set $U = T_{<i_{k}} \cup W$. Observe that in both cases $U \cup X$ is of size $k$. Then, $U \cup X$ is the prefix for which the algorithm aims to prove that it is a Condorcet winning team. See Figure \ref{fig:cut-algo-XY} for an illustration of the two cases.




Now, the algorithm aims to reason about all possible responses to $U \cup X$, that is, teams from $[n] \setminus U \setminus X$. First, observe that $Y$ is guaranteed to be within the \emph{best response} towards $U \cup X$. Hence, the algorithm will reason about all subsets of size $k - |Y|$ from $[n] \setminus U \setminus X \setminus Y$. More precisely, it aims to show that for every set $V \subseteq [n] \setminus U \setminus X\setminus Y$ of this size, there exists at least one pair of nodes $u \in U$ and $v \in V$ such that \begin{equation}
    v(u) - v(v) > |v(X) - v(Y)|. \label{eq:condBound}
\end{equation}
%Observe that we can assume wlog that $Y \subseteq V$ as this will is the case in a best response. 
This suffices to prove the claim that $U$ is a Condorcet winning team since $U \triangleright V$. See Figure \ref{fig:cut-algo-prove} for an illustration of the argument. 

\begin{figure}
    \centering
    \includegraphics[scale=.15]{src/figures/fig2.jpg}
    \caption{Caption}
    \label{fig:cut-algo-prove}
\end{figure}

%TODO Explain list
There are two ways in order to prove this claim: Either, the algorithm is lucky and is able the show that there exists $u \in U$ and $v \in T_{<i_{2k}} \setminus U \setminus X \setminus Y$ for which (\ref{eq:condBound}) holds. In this case, it is done since $v$ is guaranteed to be within the best response towards $U \subseteq X$. For the other case, the algorithm introduces a list $L$ where is saves all the nodes from $[n] \setminus U \setminus X \setminus Y$ for which it has already shown that \ref{eq:condBound} holds. When this list becomes larger than $|T_{\leq i_{2k}}| - 2k + 1$ then it is guaranteed that the best response towards $U \cup X$ contains at least one node from the list $L$. 




\begin{algorithm}[tb] 
\begin{algorithmic}[1]
\STATE \textbf{Input: } a partition of $[n]$ into $T_1 \triangleright T_2 \triangleright \dots \triangleright T_{\ell}$ with $i_{k} \neq i_{2k}$ ($i_k$ and $i_{2k}$ defined as in the text)
\STATE \textbf{Output: } a CondorcetWinning Team \\
\smallskip
\STATE $j \leftarrow \min \{k - |T_{<i_k}|, |T_{\leq i_k}| - k\}$
\STATE Set $X$ and $Y$ to be two disjoint, $j$-sized subsets of $T_{i_k}$
\STATE Set $W \leftarrow T_{i_k} \setminus X \setminus Y$
\STATE Set $L \leftarrow \emptyset$
\STATE $(*)$ Set $Z$ to be a subset of $T_{i_{2k}}\setminus L$ of size $2k - |T_{<i_{2k}}|$
\WHILE{$|L|< |T_{\leq i_{2k}}| - 2k + 1$}
\IF{$|T_{\leq i_k}| - k<k-|T_{<i_k}|$}
\STATE $U \leftarrow T_{<i_k} \cup W, \;V \leftarrow (T_{>i_k} \cap T_{<i_{2k}}) \cup Z$ \\ 
\ELSE \STATE $U \leftarrow T_{<i_k}, \; V \leftarrow W \cup (T_{>i_k} \cap T_{<i_{2k}}) \cup Z$ \\
\ENDIF
%\IF{$(U \cup X \succ V \cup Y)$ and $(U \cup Y \succ V \cup X)$}
\IF{$V \cup Y \succ U \cup X$ or $V \cup X \succ U \cup Y$} \label{line:firstquery}
\STATE \textbf{return} $\mathrm{CondorcetWinning}(\mathrm{refinedPartition})$\label{line:partition1}
\ENDIF
\STATE $(u,v),(S,S') \leftarrow \mathrm{WarmStartUncover}(U,V,X,Y)$ \label{line:warmstart1}
\IF{$\mathrm{Compare}((u,v),(S,S'),(X,Y))$ not true}
\STATE \textbf{return} $\mathrm{CondorcetWinning}(\mathrm{refinedPartition})$ \label{line:partition2}
\ENDIF
\IF{$v \in Z$}
\STATE $L \leftarrow L \cup \{v\}$, go to $(*)$
\ELSE \STATE \textbf{return} $U \cup X$ \label{line:return1}
\ENDIF
%\ELSE \STATE $(x,y),(S,S') \leftarrow \mathrm{Compare}((u,v),(S,S'),(X,Y))$ \\ 
%\STATE $\mathcal{T} \leftarrow \mathrm{NewCut}(\mathcal{T},(x,y),(S,S'))$
%\STATE \textbf{return} $\mathrm{CondorcetWinning}(\mathcal{T})$
%\ENDIF
%\ENDIF
%\ELSE \STATE wlog $(U \cup X \succ V \cup Y)$ and $(V \cup X \succ U \cup Y)$
%\STATE $(x,y),(S,S') \leftarrow \mathrm{WarmStartUncover}(X,Y,U,V)$
%\STATE $\mathcal{T} \leftarrow \mathrm{NewCut}(\mathcal{T},(x,y),(S,S'))$
%\STATE \textbf{return} $\mathrm{CondorcetWinning}(\mathcal{T})$
%\ENDIF
\ENDWHILE
\STATE \textbf{return} $U \cup X$ \label{line:return2}
\end{algorithmic}
\caption{CordorcetWinning}\label{alg:condorcet1}
\end{algorithm}



 
\begin{proposition}\label{thm:CondorcetWiningCase1}
Algorithm \ref{alg:condorcet1} works correctly. In particular, all statements are well-defined, in line \ref{line:partition1} and \ref{line:partition2} a refined partition can be constructed, and the returned team is a Condorcet winning team. 
\end{proposition}

\begin{proof}
We start by showing that the two duels in line \ref{line:firstquery} (I mean line 14) are feasible. To this end observe that $U,V,X$ and $Y$ are disjoint by construction. To argue about their cardinalities, we consider the two cases of the if condition. First, assume $|T_{\leq i_k}| - k < k - |T_<i_k|$. Then \[|U| = |T_{<i_k}| + |T_{i_k}|-2j = |T_{\leq i_k}| - (|T_{\leq i_k}| - k) - j = k-j.\] As $|X|=|Y|=j$, we get that $|U|+|X|=|U|+|Y|=k$. Similarly, we have \[|V| = |T_{<i_{2k}}| - |T_{\leq i_k}| + |Z| = |T_{<i_{2k}}| - |T_{\leq i_k}| + 2k = |T_{<i_k}| = k + k - |T_{i_{k}}| = k - j.\] Hence, also $|U|+|X|=|U|+|Y|=k$.

Next, we show that we can find a refined partition in line \ref{line:partition1} (I mean 15). Assume wlog that $V \cup Y \succ U \cup X$ holds and observe that both statements cannot be true as $U \triangleright V$ by construction. Hence, we have $U \cup Y \succ V \cup X$ which implies that we can call $\mathrm{WarmStartUncover(Y,X,U,V)}$ which returns a pair $(y,x)$ as well as a witness from $\mathcal{S}_{y,x}$. Since $x$ and $y$ are from the same indifference class of $\mathcal{T}$, namely $T_{i_k}$, we can call the $\mathrm{NewCut}$ subroutine and obtain a refined partition. 

The call to $\mathrm{WarmStartUncover}$ in line \ref{line:warmstart1} (I mean 17) is feasible, as the non-satisfaction of the if condition implies that $U \cup X \succ V \cup Y$ and $U \cup Y \succ V \cup X$. 

In line \ref{line:partition2} (I mean 19) we can refine the partition $\mathcal{T}$, as, if $\mathrm{Compare}((u,v),(S,S'),(X,Y))$ does not return true, it returns a pair $(x,y)$ with $x \in X$ and $y \in Y$ (or $(y,x)$) together with a witness from $\mathcal{S}_{xy}$ (or $\mathcal{S}_{yx}$). Since $x$ and $y$ are both from the same indifference class of $\mathcal{T}$, namely $T_{i_k}$, we can refine $\mathcal{T}$ by calling the $\mathrm{NewCut}$ subroutine. 

Lastly, we show that $U \cup X$ is a Condorcet winning team when the algorithm reaches line \ref{line:return1} or line \ref{line:return2} (I mean 24 or 27). We first discuss line 24. First, observe that $U \triangleright V, u \in U$, $v \in V$ and $(S,S')$ is a witness for their relation, that is, $(S,S') \in \mathcal{S}_{uv}$. Moreover, since $\mathrm{Compare}((u,v),(S,S'),(X,Y))$ is true, we know that 
\begin{equation}
v(u) - v(v) > |v(X) - v(Y)|. \label{eq:compareuvXY}
\end{equation} Additionally we know that $v \in V \setminus Z$, which implies that $v \in T_{<i_{2k}}$. Hence, $v$ is in particular contained in the best response against $U \cup X$. Since $Y$ is also guaranteed to be within the best response, we can denote the best response by $V' \cup Y$. Using \cref{eq:compareuvXY} and the fact that $U \triangleright V'$, we get 
\begin{align*}
    v(U \cup X) - v(V' \cup Y) &= v(U \setminus \{u\}) + v(u) + v(X) - v(V' \setminus \{v\}) - v(v) - v(Y) \\ 
    & > v(U \setminus \{u\}) - v(V' \setminus \{v\}) > 0, 
\end{align*}
showing that $U \cup X \succ V' \cup Y$. 

Now, consider the situation in line \ref{line:return2} (I mean 27). This implies that the list $L$ is of length $|T_{\leq i_{2k}}| - 2k +1$ and for each $v \in L$ there exists $u \in U$ such that \begin{equation} v(u) - v(v) > |v(X) - v(Y)|. \label{eq:compareuvXY2}\end{equation} Again, the best response against $U \cup X$ contains $Y$. Denote the best response by $V' \cup Y$. By the size of $L$ we know that $V' \cap L \neq \emptyset$. Let $v$ be a node in the intersection and $u$ be the node for which the algorithm has proven \cref{eq:compareuvXY2}. Due to the same argumentation as before, $U \triangleright V'$ and $v(u') - v(v') > v(X) - v(Y)$ implies $U \cup X \succ V' \cup Y$. 
\end{proof}

\begin{proposition}
Algorithm \ref{alg:condorcet1} terminates after performing $\mathcal{O}(k^3)$ duels. 
\end{proposition}




\subsection*{Algorithm: CondorcetWinning - Case 2}


%Write some fluffy text for algorithm 

In the following we consider the case when we are confronted with a weak ordering partition $\mathcal{T}$ for which $i_k = i_{2k}$ holds. In other words, the set $T_{i_k}$ contains players which belong to $[k]$ as well as players not belonging to $[2k]$. This situation requires a more sophisticated approach to find and especially prove that a given team is a Condorcet winning team. Before we describe the approach formally within Algorithm \ref{alg:condorcet2}, we give the high level idea upfront. 

The algorithm start by partitioning the set $T_{\leq i_{2k}}$ into six sets $U_1,U_2,X,Y,W_1,W_2,$ and $Z$, where the only known relationships are that $(U_1 \cup U_2) \triangleright (X \cup Y \cup W_1 \cup W_2 \cup Z)$. Regarding the sizes of the sets it holds that $|U_i| = |W_i|$ for $i \in \{1,2\}$, $|X|=|Y|$ and $|U_1| = |Z|$. See Figure \ref{fig:fig3} for an illustration of the situation. 


\begin{figure}
    \centering
    \includegraphics[scale=.3]{src/figures/fig3.png}
    \caption{Caption}
    \label{fig:fig3}
\end{figure}

Now, the main aim of the algorithm will be to define some $0< \epsilon_1 < \epsilon_2$ and prove that the following statements are true: 

\begin{enumerate}[label=(\roman*)]
    \item $|v(X) - v(Y)| < \epsilon_1$,  %\label{it:diffXY}
    \item $|v(a) - v(b)| < \epsilon_2$ for all $a \in Y \cup W$ and $b \in Z$, and % \label{it:diffaz}
    \lc{which $W$?}
    \item there exist $u_1, \dots, u_{|Z|} \in U_1 \cup U_2$ as well as $w_1, \dots, w_{|Z|} \in W_1 \cup W_2$ such that 
    \begin{itemize}
        \item $v(u_1) - v(w_1) \geq \epsilon_1$
        \item $v(u_i) - v(w_i) \geq \epsilon_2$ for all $i \in \{2, \dots, |Z|\}$
    \end{itemize}
\end{enumerate}

\begin{figure}
    \centering
    \includegraphics[scale=.4]{src/figures/fig4.png}
    \caption{Caption}
    \label{fig:fig4}
\end{figure}

With the help of these three statements we can show that $U_1 \cup U_2 \cup X$ is a Condorcet winning team. More precisely, one can show that $v(U_1 \cup U_2 \cup X) - v(W_1 \cup W_2 \cup Y) > |Z| \cdot \epsilon_2$ and $v(W_1 \cup W_2 \cup Y) - v(B^*) > - |Z| \cdot \epsilon_2$, where $B^*$ is the best response towards $U_1 \cup U_2 \cup X$. Clearly, this suffices to show that $U_1 \cup U_2 \cup X$ is Condorcet winning. 


For an illustration of the argument see Figure \ref{fig:fig4}, for details see the proof of Proposition \ref{thm:CondorcetWinning2}. 


If the algorithm is not able to show these statements directly, then it will be able to refine the partition $\mathcal{T}$. This can either lead to calling itself again or producing a situation in which Algorithm \ref{alg:condorcet1} can be applied.  


\begin{algorithm}[tb] 
\begin{algorithmic}[1]
\STATE \textbf{Input: } a partition of $[n]$ into $T_1 \triangleright T_2 \triangleright \dots \triangleright T_{\ell}$ with $i_{k} = i_{2k}$ ($i_k$ and $i_{2k}$ defined as in the text)
\STATE \textbf{Output: } a CondorcetWinning Team \\
\smallskip
%\STATE $j \leftarrow k - |T_{<i_k}|$
\STATE Set $U \leftarrow T_{<i_k}$
\STATE Set $X$ and $Y$ to be two disjoint, $(k-|U|)$-sized subsets of $T_{i_k}$
\STATE Set $W$ to be a $|U|$-sized subset of $T_{i_k} \setminus X \setminus Y$
\STATE Set $Z$ to be $T_{i_k} \setminus X \setminus Y \setminus W$
\STATE Set $W_1$ to be a $|Z|$-sized subset of $W$ and $W_2 \leftarrow W \setminus W_1$
\STATE Set $U_1$ to be a $|Z|$-sized prefix of $U$ and $U_2 \leftarrow U \setminus U_1$
\IF{$W_2 \cup (Y \cup W_1) \succ U_2 \cup (X \cup Z)$ or $ W_2 \cup (X \cup Z)\succ U_2 \cup (Y \cup 
W_1)$} \label{line:firstIF}
\STATE {\textbf{return} $\mathrm{CondorcetWinning(refined Partition)}$} \label{line:part1}
\ENDIF
\STATE $(\bar{u},\bar{w}),(S,S') \leftarrow \mathrm{WarmStartUncover(U_2,W_2,(X \cup Z),(Y \cup W_1))}$ \label{line:warmstart}
\STATE Let $\bar{T}$ be indifference class of $\bar{u}$ in $\mathcal{T}$
\FOR{$u \in \bar{T} \cap U_1 \cup \{\bar{u}\}$}
\FOR{$w \in W_1 \cup \{\bar{w}\}$}
\STATE $S'' \leftarrow f_{\bar{w},w}(S')$ 
\IF{$(S,S'') \not \in \mathcal{S}_{u,w}$}
\STATE {\textbf{return} $\mathrm{CondorcetWinning(refined Partition)}$} \label{line:part2}
\ENDIF
\IF{$\mathrm{Compare}((u,w),(S,S''),(X,Y))$ not true}
\STATE {\textbf{return} $\mathrm{CondorcetWinning(refined Partition)}$} \label{line:part3}
\ENDIF
\FOR{$z \in Z$}
\FOR{$q \in S'' \cap (W \cup Y)$}
\IF{$\mathrm{Compare}((u,w),(S,S''),(\{z\},\{q\}))$ not true} \label{line:comparezq}
\STATE {\textbf{return} $\mathrm{CondorcetWinning(refined Partition)}$} \label{line:part4}
\ENDIF
\ENDFOR
\ENDFOR
\STATE $(Q,Q') \leftarrow (S \setminus Z \cup f_{w^*,w}(W_1), S'' \setminus f_{w^*,w}(W_1) \cup Z)$
\IF{$(Q,Q') \not \in S_{u,w}$}
\STATE {\textbf{return} $\mathrm{CondorcetWinning(refined Partition)}$} \label{line:part5}
\ENDIF
\FOR{$z \in Z$}
\FOR{$w' \in Q \cap W_2$}
\IF{$\mathrm{Compare}((u,w),(Q,Q'),(\{w'\},\{z\}))$ not true} \label{line:comparezq2}
\STATE {\textbf{return} $\mathrm{CondorcetWinning(refined Partition)}$} \label{line:part6}
\ENDIF
\ENDFOR
\ENDFOR
\ENDFOR
\ENDFOR
\STATE \textbf{return} $U \cup X$
\end{algorithmic}
\caption{CordorcetWinning}\label{alg:condorcet2}
\end{algorithm}

\begin{proposition} \label{thm:CondorcetWinning2}
Algorithm \ref{alg:condorcet2} works correctly. In particular, all statements are well-defined, in line \ref{line:part1},\ref{line:part2},\ref{line:part3},\ref{line:part4},\ref{line:part5}, and \ref{line:part6}, a refined partition can be constructed, and the returned team is a Condorcet winning team. 
\end{proposition}

\begin{proof}
\textbf{Part I.} We show the first two statements by going through the algorithm line by line. 

We start by showing that in line \ref{line:firstIF} (I mean line 9), the two queries are feasible. First observe that by construction, the sets $U_1,U_2,X,Y,W_1,W_2,$ and $Z$ are disjoint. Moreover, $|U| = |W|$, $|U_1| = |W_1|$, and hence $|U_2| = |W_2|$. Also, $|X|=|Y|$ and $|W_1| = |Z|$. In total, we get that $|W_2| + |Y| + |W_1| = |U_1| + |X| + |Z| = |U|+|X| = k$ and the same holds for the other query as well. 

Next, we show that in line \ref{line:part1} (I mean line 10), the partition $\mathcal{T}$ can indeed be refined. Consider wlog the case when $W_2 \cup (Y \cup W_1) \succ U_2 \cup (X \cup Z)$. Then, since $U_2 \triangleright W_2$ we know that $U_2 \cup (Y \cup W_1) \succ W_2 \cup (X \cup Z)$ needs to hold. Hence, $\mathrm{WarmStartUncover}(Y\cup W_1,X \cup Z,W_2,U_2)$ returns a pair $(a,b)$ with $a \in Y \cup W_1$ and $b \in X \cup Z$ together with a witness $(S,S') \in \mathcal{S}_{a,b}$. Since $a,b \in T_{i_k}$, we can call $\mathrm{NewCut}(\mathcal{T},(a,b),(S,S'))$ which returns a refined partition. An analogous argument holds for the case $W_2 \cup (X \cup Z) \succ U_2 \cup (Y \cup W_2)$. 

We turn to show that the input for the $\mathrm{WarmStartUncover}$ subroutine is valid in line \ref{line:warmstart} (I mean 12). Since the condition in line \ref{line:part1} (I mean 9) is not satisfied, we know that $U_2 \cup (X \cup Z) \succ W_2 \cup (Y \cup W_1)$ and $U_2 \cup (Y \cup W_1) \succ W_2 \cup (X \cup Z)$. This suffices to show that $(U_2, W_2,(X \cup Z),(Y \cup W_1))$ is a valid input for $\mathrm{WarmStartUncover}$. Hence, for the returned pair $(\bar{u},\bar{w})$ is holds that $\bar{u} \in U_2$ and $\bar{w} \in W_2$. Moreover, we can assume in the following wlog that $(X \cup Z) \subseteq S$ and $(Y \cup W_1) \subseteq S'$. 

We continue with the situation in line \ref{line:part2} (I mean 18) and show that a refined partition can be found. We distinguish two cases. 

\textbf{Case 1} $(S,S'') \in \mathcal{S}_{\bar{u},w}$. This implies $(i) \; S \cup \{\bar{u}\} \succ S'' \cup \{w\}$ and $(ii) \; S'' \cup \{\bar{u}\} \succ S \cup \{w\}$. Moreover, from $(S,S'') \not \in \mathcal{S}_{u,w}$ we know that either $ (iii) \; S \cup \{w\} \succ S'' \cup \{u\} $ or $ (iv) \;S'' \cup \{w\} \succ S \cup \{u\}$ is true. Assume without loss of generality that $(iii)$ holds. Then, together with $(ii)$ we get that $S'' \cup \{\bar{u}\} \succ S \cup \{w\} \succ S'' \cup \{u\}$, hence $\bar{u} \succ u$ and in particular $(S \cup \{w\},S'') \in \mathcal{T}_{\bar{u},u}$. Since $\bar{u}$ and $u$ are from the same indifference class of $\mathcal{T}$, calling $\mathrm{NewCut2}(\mathcal{T},(\bar{u},u),(S \cup \{w\},S''))$ returns a refined partition. An analogous argument holds when $(iv)$ is true.   


\textbf{Case 2} $(S,S'') \not\in \mathcal{S}_{\bar{u},w}$. Then, either $(i)\; S \cup \{w\} \succ S'' \cup \{\bar{u}\}$ or $(ii) \; S'' \cup \{w\} \succ S \cup \{\bar{u}\}$ holds while both is not possible as $\bar{u} \succ w$. %Moreover, from $(S,S'') \not \in \mathcal{S}_{u,w}$ we know that either $ (iii) \; S \cup \{w\} \succ S'' \cup \{u\} $ or $ (iv) \;S'' \cup \{w\} \succ S \cup \{u\}$ is true. First assume that $(i)$ holds. 
First, assume $(i)$ is true. Then, from $(S,S') \in \mathcal{S}_{\bar{u},\bar{w}}$, we know that $(iii) \; S' \cup \{\bar{u}\} \succ S \cup \{\bar{w}\}$. Reformulating $(i)$ to $S \cup \{w\} \succ S' \setminus \{w\} \cup \{\bar{u}\} \cup \{\bar{w}\}$ and $(iii)$ to $S' \setminus \{w\} \cup \{\bar{u}\} \cup \{w\} \succ S \cup \{\bar{w}\}$ shows that $w \succ \bar{w}$ and in particular $(S,S' \setminus \{w\} \cup \{\bar{u}\}) \in \mathcal{S}_{w,\bar{w}}$. As $w$ and $\bar{w}$ are contained in the same indifference class of $\mathcal{T}$, calling $\mathrm{NewCut}(\mathcal{T},(w,\bar{w}),(S, S' \setminus \{w\} \cup \{\bar{u}\}))$ refines the partition. Second, assume that $(ii)$ holds. However, from $(S,S') \in \mathcal{S}_{\bar{u},\bar{w}}$ we know that $(iv) \; S \cup \{\bar{u}\} \succ S' \cup \{\bar{w}\}$ is true. As $S'' \cup \{w\} = S' \cup \{\bar{w}\}$ this yields a contradiction to $(ii)$. 

We turn to prove that we can find a refined partition within line \ref{line:part3} (I mean line 21). When $\mathrm{Compare}((u,w),(S,S''),(X,Y))$ is not true, then it returns a pair $(x,y)$ with $x \succ y$ (or vice versa) and a witness $(P,P') \in \mathcal{S}_{x,y}$ (or $(P,P') \in \mathcal{S}_{y,x}$). Since $x$ and $y$ are from the same indifference class of $\mathcal{T}$, namely $T_{i_k}$, the algorithm can call $\mathrm{NewCut}(\mathcal{T},(x,y),(P,P'))$ and obtain a refined partition. 

We continue with the situation in line \ref{line:part4} (I mean line 28). When $\mathrm{Compare}((u,w),(S,S''),(\{z\},\{w'\}))$ is not true, then it returns a pair $(z,w')$  (or $(w',z)$) and a witness $(P,P') \in \mathcal{S}_{z,w'}$ (or $(P,P') \in \mathcal{S}_{w',z}$). Since $z$ and $w'$ are from the same indifference class of $\mathcal{T}$, namely $T_{i_k}$, the algorithm can call $\mathrm{NewCut}(\mathcal{T},(z,w'),(P,P'))$ and obtain a refined partition.

We turn to prove that we can find a refined partition within line \ref{line:part5} (I mean 32). From $(Q,Q') \not\in \mathcal{S}_{u,w}$ we know that either $(i) \; Q \cup \{w\} \succ Q' \cup \{u\}$ or $(ii) \; Q' \cup \{w\} \succ Q \cup \{u\}$ while both are not possible as $u \succ w$. First, assume that $(i)$ holds. From $(S,S'') \in \mathcal{S}_{u,w}$ we get in particular that $(iii) \; S'' \cup \{u\} \succ S \cup \{w\}$ holds. Rewriting $(i)$ as $f_{\bar{w},w}(W_1) \cup S \setminus Z \cup \{w\} \succ Z \cup S'' \setminus f_{\bar{w},w}(W_1) \cup \{u\}$ and $(iii)$ as $f_{\bar{w},w}(W_1) \cup S'' \setminus f_{\bar{w},w}(W_1) \cup \{u\}\succ Z \cup S \setminus Z   \cup \{w\}$ establishes that we can call $\mathrm{WarmStartUncover}(f_{\bar{w},w}(W_1),Z,S'' \setminus f_{\bar{w},w}(W_1) \cup \{u\},S \setminus Z \cup \{w\} )$ which returns a pair $(\hat{w},\hat{z})$ with $\hat{w} \in f_{\bar{w},w}(W_1)$ and $\hat{z} \in Z$ together with a witness for their relation. As $\hat{w}$ and $\hat{z}$ are from the same indifference class of $\mathcal{T}$ we can call $\mathrm{NewCut}$ to refine the partition. The case when $(ii)$ follows by an analogous argument. 

Lastly, we turn to show that we can find a refined partition within line \ref{line:part6} (I mean 37). To see that $\mathrm{Compare}((u,w),(Q,Q'),(\{w'\},\{z\}))$ is a valid query, observe that $w' \in Q$ and $z \in Q'$. Moreover, $(Q,Q') \in \mathcal{S}_{u,w}$. Hence, $\mathrm{Compare}$ returns the pair $(w',z)$ (or $(z,w')$) together with a witness from $\mathcal{S}_{w',z}$ (or $\mathcal{S}_{z,w'}$). As $z$ and $w'$ are from the same equivalence class of $\mathcal{T}$, we can call the $\mathrm{NewCut}$ and obtain a refined partition.   

\textbf{Part II.} We now show that the set returned by $\mathrm{CondorcetWinning(\mathcal{T})}$ is indeed a Condorcet winning team. If, at some point of the algorithm $i_k \neq i_{2k}$, then the statement follows from Theorem \ref{thm:CondorcetWiningCase1}. Otherwise, the algorithm returns $U \cup X$ which implies that within the last call of $\mathrm{CondorcetWinning}$ none of the if condition was satisfied. We show in the following that this implies that $U \cup X$ is a Condorcet winning team. 

We define 
\begin{align*}
w^*_1 &= \argmax_{w \in W_1 \cup \{\bar{w}\}} v(w), \\ 
w_2^* &= \argmax_{w \in W_1 \cup \{\bar{w}\} \setminus \{w_1^*\}} v(w), \text{ and } \\ u^* &= \argmin_{u \in \bar{T} \cap U_1} v(u).
\end{align*}
Moreover, $\epsilon_1 = v(u^*) - v(w^*_1) \text{ and } \epsilon_2 = v(u^*) - v(w^*_2)$. 

We claim that 
\begin{enumerate}[label=(\roman*)]
    \item $|v(X) - v(Y)| < \epsilon_1$, and \label{it:diffXY}
    \item $|v(a) - v(b)| < \epsilon_2$ for all $a \in Y \cup W$ and $b \in Z$. \label{it:diffaz}
\end{enumerate}

For \ref{it:diffXY} observe that there was a point within the iteration of the algorithm when $u = u^*$ and $w=w^*_1$. Moreover, the algorithm called $\mathrm{Compare}((u,w),(S,S''),(X,Y))$ which returned true. As we have argued for the subroutine $\mathrm{Compare}$, this implies $\epsilon_1 = v(u^*) - v(w^*_1) > |v(X) - v(Y)|$.

To show \ref{it:diffaz}, we distinguish three cases. Let $a \in Y \cup W$ and $z \in Z$. 

\textbf{Case 1.} $a = w_1^*$. Then, there was a point within the iteration of the algorithm when $u=u^*, w=w_2^*, q = w_1^*=a$ and $z = b$. As $\mathrm{Compare}((u,w),(S,S'),(\{z\},\{q\}))$ returned true in line \ref{line:comparezq} (I mean 25), we know that \[|v(a)- v(b)| < v(u^*)-v(w^*_2) = \epsilon_2.\] 

\textbf{Case 2.} $a \neq w_1^*, a \in S$. Then, there was a point within the iteration of the algorithm when $u=u^*, w=w_1^*, q = a$ and $z = b$. As $\mathrm{Compare}((u,w),(S,S'),(\{z\},\{q\}))$ returned true in line \ref{line:comparezq} (I mean 25), we know that \[|v(a)- v(b)| < v(u^*)-v(w^*_1) = \epsilon_1 < \epsilon_2.\] 

\textbf{Case 3.} $a \neq w_1^*, a \in S'$. Then, there was a point within the iteration of the algorithm when $u=u^*, w=w_1^*, q = a$ and $z = b$. As $\mathrm{Compare}((u,w),(Q,Q'),(\{z\},\{q\}))$ returned true in line \ref{line:comparezq2} (I mean 37), we know that \[|v(a)- v(b)| < v(u^*)-v(w^*_1) = \epsilon_1 < \epsilon_2.\] 
 
Lastly, we show that \ref{it:diffXY} and \ref{it:diffaz} suffice to prove that $U \cup X$ is a Condorcet winning team. To this end let $B^*$ be the best response against $U \cup X$. Observe that $B^* \subseteq Y \cup W \cup Z$. 

We start by showing 
\begin{align*}
    v(U \cup X) - v(W \cup Y) & = v(U_1 \cup \{\bar{u}\} \setminus \{u^*\}) + v(u^*) + v(U_2 \setminus \{\bar{u}\}) +v(X) - v(w^*_1) - v(W_1 \cup \{\bar{w}\} \setminus \{w^*_1\}) - v(W_2 \setminus \{\bar{w}\}) - v(Y) \\ 
    & = v(X) - v(Y) + v(u^*) - v(w^*_1) +  v(U_1 \cup \{\bar{u}\} \setminus \{u^*\}) - v(W_1 \cup \{\bar{w}\} \setminus \{w^*_1\}) + v(U_2 \setminus \{\bar{u}\}) - v(W_2 \setminus \{\bar{w}\}) \\ 
    & > - \epsilon_1 + v(u^*) - v(w^*_1) +  v(U_1 \cup \{\bar{u}\} \setminus \{u^*\}) - v(W_1 \cup \{\bar{w}\} \setminus \{w^*_1\}) + v(U_2 \setminus \{\bar{u}\}) - v(W_2 \setminus \{\bar{w}\}) \\ 
    & > - \epsilon_1 + \epsilon_1 +  v(U_1 \cup \{\bar{u}\} \setminus \{u^*\}) - v(W_1 \cup \{\bar{w}\} \setminus \{w^*_1\}) + v(U_2 \setminus \{\bar{u}\}) - v(W_2 \setminus \{\bar{w}\}) \\
    & > - \epsilon_1 + \epsilon_1 + |Z| \cdot \epsilon_2 + v(U_2 \setminus \{\bar{u}\}) - v(W_2 \setminus \{\bar{w}\}) \\
    & > - \epsilon_1 + \epsilon_1 + |Z| \cdot \epsilon_2 + 0 \\ 
    & = |Z| \cdot \epsilon_2.
\end{align*}
The first inequality follows by \ref{it:diffXY}, the second by the definition of $\epsilon_1$, the third by the definition of $\epsilon_2$ and the fact that $|u(U_1 \cup \{\bar{u}\} \setminus \{u^*\})| = |v(W_2 \cup \{\bar{w}\} \setminus \{w_1^*\})| = |Z|$, and the last by the fact that $U_2 \triangleright W_2$. 

In addition, we get 

\begin{align*}
    v(W \cup Y) - v(B^*) & = v(W \cup Y \setminus B^*) - v(B^* \cap Z) \\ 
    & > - |Z| \cdot \epsilon_2, 
\end{align*}
where the inequality follows from the fact that $|v(W \cup Y)| = |v(B^* \cap Z)| < |Z|$ and \ref{it:diffaz}. 

Summing up the two inequalities yields \[v(U \cup X) - v(B^*) > 0,\]
which concludes the proof. 
\end{proof}



\begin{proposition}
Algorithm \ref{alg:condorcet2} terminates after $\mathcal{O}(k^5)$ queries.
\end{proposition}

==> src/intro_ICML.tex <==
Multi-arm bandits (MAB) is a classical model of decision making under uncertainty. 
Although the simplicity of the model, it already incorporates the essential tradeoff between exploration and exploitation. In MAB, the learner performs actions and can only observe rewards of the actions performed. There are two classical tasks in MAB, the first is \emph{regret minimization}, in which the learner's cumulative reward is compared to that of the best action, and \emph{best arm identification}, where the goal is to identify a near-optimal action while minimizing the number of actions executed. The MAB has numerous practical applications, from online advertising, recommendation systems, clinical trials, and more. (See \cite{Slivkins-book,Lattimore-Szepesvari-Book} for more background on MAB).

One weakness of the MAB model is the assumption that  real-valued rewards are always available. In many applications, it is more natural to compare two actions and observe which one of them is better rather than give every  single action a numerical reward. For example, recommendation systems often suggest two items and obtain only their relative preference as feedback (e.g., by a click on one of them). This leads very naturally to the well-known model of dueling bandits \cite{Yue2012}, where the learner selects a pair of actions each time and observes the binary outcome of a duel between them. See \cite{Busa2018} for survey on the extensions of this model.

In this work we are interested in the case that the learner has to select two disjoint subsets of actions, each of size $k>1$, called \textit{teams}, for a duel. 
This appears naturally in many applications. Our setting includes for example online advertisements where multiple products are bundled to a single display ad and a customer can click on any of two presented bundles. Another example are online games offering in-app bundle purchases, where the information about the sales of different bundles can be used to improve the composition of the bundles. Moreover, in (online) sports, a trainer seeks to identify a best team from a set of players by observing the outcomes of matches. In tennis double and relay races, each match requires two disjoint teams of players to compete. Similar phenomena appear in many team sports and even in working environments, where different R\&D teams compete on implementing a project.  

Our basic model is the following. We have a universe of $n$ players, and at each time the learner selects two disjoint teams for a duel and observe the winner. For any two different teams, there exists an unknown stationary probability that determines the winner of a duel between them. %(We assume that probabilities 
%of different teams 
%are bounded away from $1/2$ by a parameter $\theta>0$.)
The goal of the learner is to minimize the number of duels required to identify, with high probability, a \textit{Condorcet winning team}, i.e., a team which 
wins against any other disjoint team (with a probability of at least $1/2$).
We do assume a total order on all teams which implies the existence of a Condorcet winning team, yet it is not necessarily unique. We make a minimal assumption on this total order among teams, namely, that it is \emph{consistent} to some total order among the players. \sti{Moreover, we impose the assumption of \emph{Strong Stochastic Transitivity} on the probabilistic comparisons, which is very natural in dueling bandit settings.}
%
% Our assumptions imply that there is a linear order between the players. 

Clearly, given the total order among the players, the best team is the one that contains the top $k$ players. %, however the learner has to deduce it from team duels. 
However, relations between players and in particular the team of the top $k$ players might not be deducible from observations (i.e., the latent winning probabilities between all disjoint teams duels provide proof for their relation). Consider for example an instance with four players $1\succ2\succ3\succ4$ where $k=2$ and the total order among the teams is lexicographical, i.e., $12\succ13\succ14\succ23\succ 24\succ34$. Then, there exist only three feasible duels, each of which is won by the team containing player $1$. If all three feasible duels are won with equal probability, the learner has no chance of detecting the team $12$ as the top $k$ team. However, any of the teams $12,13$ and $14$ is a Condorcet winning team. 

We consider two settings, a deterministic setting, where outcomes of duels are deterministic, thus for each pair duel between two teams one of them is always the winner, and a stochastic setting, where the outcomes are probabilistic. We develop algorithms for each. Our main goal is to have the number of duels to be polynomial in the number of players $n$ and team size $k$, although the number of teams is exponential in $k$, i.e., $\Omega((\frac{n}{k})^k)$ and the number of valid duels is $\Omega(2^k(\frac{n}{2k})^{2k})$.


We introduce a gap parameter $\Delta_{i,j}$, which is the difference between the probabilities that a random team, which includes player $i$, is better than a random team, which includes player $j$. 
%\footnote{\red{USK: This is not true, right? It is the probability that a player $i$ is in a better team than $j$ when they are paired with random disjoint subsets of size $k-1$.}\blue{YM: I corrected it, take a look}\red{I am not sure what we mean by "probability to win" mean. Is this dependent on the "P Matrix"? If so, then this should be our old bug since the Z's and hence also the $\Delta$ only depends on the linear order and not the P values.}} 
Our main interest is $\Delta=\Delta_{k,k+1}$, which is the gap parameter between the $k$ and $(k+1)$ top players. We show, using the total order between teams and consistency\sti{and strong stochastic transitivity} that  this implies that $\Delta_{i,j}\geq \Delta$ for any player $i$ which is among the top$-k$ and any player $j$ which is not among the top$-k$. (For other pairs of players we do not deduce any bound on $\Delta_{i,j}$.)

%(For other pairs of players we do not deduce such relationship.)

For the deterministic setting, we derive two algorithms. Our first is a gap-dependent algorithm that requires  $\mathcal{O}(nk\log{(k)}+k\log(k)(\frac{\log \log(k)}{\Delta} + k))$ duels. Our second algorithm is gap-independent, and requires $O(nk\log{(k)}+2^{O(k)})$ duels. Both our algorithms employ an initial phase that runs in polynomial time, where the number of players is reduced from $n$ to $6k$ with the guarantee that the best $2k$ players are part of this subset. (This guarantee is deterministic.) The two algorithms differ in their search for a Condorcet winning team within this reduced instance.  

For the stochastic setting, we assume that the probability of winning, for any duel, is bounded away from $1/2$ by at least $\theta$. Given this assumption, we do a reduction from the stochastic setting to the deterministic setting,  and deduce algorithms for the stochastic setting.
%
%Our algorithm identifies a Condorcet winning team after $O(nk\log(1/\delta)/\Delta^2)$ duels with a confidence of $1-\delta$. 
%[LC: added the $\log{1/\delta}$ here]\\

Two significant challenges arise from the restrictions on which teams can be chosen for duels, that are very much aligned with our motivation. Namely, the learner can only select  disjoint teams, and the teams size, $k$, is given in advance. 
To understand these challenges, consider a learner which is allowed to duel teams with mutual players 
%(e.g., if instead of players we had items types and $n$ identical items for each type, thus the same item can play simultaneously for both dueling teams), %USK: I think the text reads better without this part
or alternatively, to determine the team size, $k$.
Such a learner would be able to either simulate single elements (players) pairwise comparisons algorithms (such as find top$-k$  or sorting) by pairing each of the elements with the same subset of size $k-1$ players or by selecting $k=2$, respectively. %\usk{why not k=1?}LC: because the problem is defined with k>1.. 
% \blue{but for $k=2$ the problem still isn't trivial, right? I think it is no problem to write $k=1$ here. Since our problem is also defined such that we cannot chose $k$}

Indeed, the inherent difficulty of the problem comes from not being able to simulate single elements comparisons. We encounter two immediate limitations in this area: (1) Not all the relations between two single players are deducible, (see example above), and (2) Even for pairs of players with deducible relation, having $\Omega(2^k(\frac{n}{2k})^{2k})$ valid duels and exactly the same amount of (latent) winning probabilities makes the task of deducing their relation hard\footnote{We stress that in contrast to dueling bandits, where the set of comparable items contains $n$ items, here we have ${n \choose k}$ comparable items.}. To overcome these issues and avoid comparing each pair of teams, we design delicate algorithms. On a high level, our algorithms first exclude as many bad players as possible. To do so, they first run a method for identifying pairwise relations between players which performs only a small number of duels but has little control over the pair for which the relation is uncovered. Subsequently, we present different approaches for identifying a Condorcet winning team within the reduced instance. 
%LC: in particular,  by assuming different PA,B for any two different disjoint pair of teams would make the problem easier as we can  %[LC: Yishay- can you please explain inside the footnote the thing you mentioned about our Deltas in our setting being $\sim 1/{n \choose k}$ while only $\sim 1/n$ in the original dueling bandits?]. 
%To overcome these issues, we design delicate algorithms that do not immediately rule out .
 %(Note that out bound is linear in $n$ and hence we do not compare each pair )
%(Note that the number of teams is $O(n^k)$.)

Due to space limitations, we relegate all proofs to the supplementary material.


\ignore{
\subsection{intro points}


* meaning of allowing equalizes between teams

\sout{- explain that in the stochastic case, all our results hold for scores as feedback (e.g., 1:3 is the duel result) by interpreting it as $z=0.25$ .}

-  define regret - future work

- provide an example for the following paragraph ``However, as previously explained, having two players $a\succ b$ does not implies there is a way for the learner to infer it, even if all the relations between disjoint teams are known. In particular, it means that we cannot assume the existence of a distinguisher for every pair of players''
% IDEA [in case we have time]: define regret, bound it by showing that we choose top - k w.h.p. 
% sort of learning one of any valid k-threshold function?

Question: is it possible to show/ give a counter example for the following claim:
if one can deduce $a\succ b$ from all the possible disjoint team comparisons then it follows that there exists a distinguisher for them. [idea: at least in the deterministic case I think that  if the winning count of a is larger then the winning count of b then it has to be due to the existence of distinguishers. if the winning counts are the same, there shouldn't be a way to distinguish them, right?]
- idea: design an instance based on the winning counts that implies a lower bound

TODO: explain why our model works for the case of transfer (link) function with values, and provide an example for a case it holds but link function doesn't:
[verify it's hold for us!] assume $A\succ B$ iff $a_1\succ \dots \succ a_k$ and $b_1\succ \dots b\succ _k$ are  lexicographic orders of $A,B$ respectively. Let $i$ be the minimal index for which $a_i\ne b_i$. then $a_i\succ b_i$ holds.
}

%1. Bandits [observe absolute values directly]
%old version
% Multi-arm bandits (MAB) is a classical model of decision making under uncertainty.
% Although the simplicity of the model, it already incorporates the essential tradeoff between exploration and exploitation. In MAB, the learner performs actions and observes only the reward of the actions performed. There are two classical tasks in MAB, the first is \emph{regret minimization}, which compares the learner cumulative reward to that of the best action, and \emph{best arm identification}, where the goal is to identify a near-optimal action while minimizing the number of actions executed. The MAB has numerous practical applications, from online advertising, recommendation systems, clinical trials and more. (See \cite{Slivkins-book,Lattimore-Szepesvari-Book} for more background on MAB).

% One weakness of the MAB model is the assumption that numerical reward can be observed. In many applications it is more natural to compare two actions rather than give a
% single action a numerical reward. For example, in recommendation systems, it is natural to compare two recommendations and decide which one is better rather than giving each recommendation a numeral  reward. This leads very naturally to the well known model of duelling bandits \cite{Yue2012}, where the learner at each time step selects a pair of actions and observes a binary outcome of a duel between them. 

% In this work we are interested in the case that the learner has to select two disjoint subsets of actions to be compared, rather than two actions. This appear naturally in many applications. For example: tennis double matches has two disjoint pairs of players compete. (A similar phenomena appears in many team sports and even in working environments, where different R\&D teams complete on implementing a project.)
% %
% Another example is two bundles of items that offered to a user, and the user selects one of the bundles. (not sure this is good, because it is not disjoint sets).

% Our basic model is the following. We have a universe of $[n]$ players and at each time the learner compares two disjoint subsets of $k$ players, called teams. For any two 
% disjoint teams there is an unknown probability that each team will win the duel between them.
% The goal of the learner is to minimize the  number of duels required to identify, with high probability, a \textit{weak Condorcet winning team}, i.e., a team which 
% wins against any other disjoint team (with probability of at least $1/2$).
% We do assume a partial order on the teams which implies the existence of a weak Condorcet winning team. 
% %
% We impose an additional natural assumptions of \emph{Strong Stochastic Transitivity} and \emph{Consistency}, which are very natural in dueling bandit settings. Our assumptions imply that there is a linear order between the players. Clearly, given the linear order the best team is the top $k$ players, but the learner has to deduce it from duels. In fact, the best team of $k$ players might not be deducible from observations. The goal of the learner is to identify some team which is a Condorcet winning team.

% We consider two settings, a deterministic setting, where the outcomes of duels are deterministic, and a stochastic setting, where the outcome is probabilistic, and develop algorithm for each. Our main goal it to have the number of dual be polynomial in the number of players $n$ and team size $k$, although the number of teams is exponential in $k$, i.e., $O(n^k)$.

% For the stochastic setting we introduce a gap parameter $\Delta_{i,j}$ which is the probability that $i$ wins against $j$, when they are extended with a random disjoint subsets of size $k-1$. Our main interest is $\Delta=\Delta_{k,k+1}$, which is the gap parameter between the $k$th and $k+1$st player. We show, using the consistency and strong transitivity and this implies that $\Delta_{i,j}\geq \Delta$ for any player $i$ which is among the top-k and any player $j$ which is not among the top-k. (For other pair of players we do not deduce any relationship.)
% %
% Our algorithm identifies the Condorcet winning team after $O(nk/\Delta^2)$ duels. 
% %
% (We remark that we cannot simulate any sorting algorithm, since in many cases we have that the comparison returns "similar". [YM: I think we should explain the cahllenegs, not sure how])
% %(Note that out bound is linear in $n$ and hence we do not compare each pair )
% %(Note that the number of teams is $O(n^k)$.)

% For the deterministic setting, we derive two algorithms. Our first is a gap-dependent algorithm that requires $O(nk\log{(k)}+k^2/\Delta)$ duels. Our second algorithm is gap-independent, and requires $O(nk\log{(k)}+2^{O(k)})$ duels. Both our algorithm employ an initial phase, where the numbers of players is reduced from $n$ to $6k$ with the guarantee that the best $2k$ players are part of this subset. (This is a deterministic guarantee.) The two algorithms differ in their search for the Condorcet winning team in this subset.  

% A significant part of the challenge arises from the fact that we can compare only disjoint teams.


\ignore{
\subsection{intro points}

[introduction]


1. Bandits [observe absolute values directly]

2. Dueling Bandits

3.Dueling Teams Bandits %[mention independent!]

3a. goal- find the k players with that together form a team with a maximal probability of defeating any other using noisy comparisons

4. Difficulty [we cannot test S+a vs. S+b directly]

5. Contributions

* meaning of allowing equalizes between teams

% todo: define query if needed?
* explain that we cannot always find a witness, and if we haven't found (and haven't tested all) we cannot know for sure that they are not..
% notation ides:
% team- $A_i$

% $\Delta(A_i,A_j), \Delta_{A_i,A_j}$


% distinguishability between two teams or players $\dis{A_i,A_j}$

% value of team or player $\val{A_i}$
% value+ weights: $\omega(C_i)/ \omega (i)$
Duel represents a match between two teams

preference elicitation, pairwise preferences

motivation ideas: math competition, R\& D teams, catch the flag, Tug of war (rope pulling), trivia, debate,  Relay race, Dodgeball, Volleyball. %dog and bone

\sout{- explain that in the stochastic case, all our results hold for scores as feedback (e.g., 1:3 is the duel result) by interpreting it as $z=0.25$ .}

-  define regret - future work

% IDEA [in case we have time]: define regret, bound it by showing that we choose top - k w.h.p. 
% sort of learning one of any valid k-threshold function?

Question: is it possible to show/ give a counter example for the following claim:
if one can deduce $a\succ b$ from all the possible disjoint team comparisons then it follows that there exists a distinguisher for them. [idea: at least in the deterministic case I think that  if the winning count of a is larger then the winning count of b then it has to be due to the existence of distinguishers. if the winning counts are the same, there shouldn't be a way to distinguish them, right?]
- idea: design an instance based on the winning counts that implies a lower bound

TODO: explain why our model works for the case of transfer (link) function with values, and provide an example for a case it holds but link function doesn't:
[verify it's hold for us!] assume $A\succ B$ iff $a_1\succ \dots \succ a_k$ and $b_1\succ \dots b\succ _k$ are  lexicographic orders of $A,B$ respectively. Let $i$ be the minimal index for which $a_i\ne b_i$. then $a_i\succ b_i$ holds.
}
